User Feedback-Informed Interface Design for Flow Management Data and Services (FMDS)

The transition to a microservices-based Flow Management Data and Services (FMDS) architecture from the existing Traffic Flow Management System (TFMS) is a critical enabler of the vision for an Information-Centric National Airspace System (NAS). The need to design a user-centric interface for FMDS is a key technical gap, as this interface connects NAS data and services to the traffic management specialists within all stakeholder groups (e.g., FAA, airlines). We provide a research-driven approach towards designing such a graphical user interface (GUI) for FMDS. Major goals include unifying the more than 50 disparate traffic management services currently hosted on TFMS, as well as streamlining the process of evaluating, modeling, and monitoring Traffic Management Initiatives (TMIs). Motivated by this, we iteratively designed a GUI leveraging human factors engineering and user experience design principles, as well as user interviews. Through user testing and interviews, we identify workflow benefits of our GUI (e.g., reduction in task completion time), along with next steps for developing a live prototype.

==> ICRAT2024_FMDS/chapters/discussion.tex <==
\section{Discussion} \label{sec:discussion}
% aMaize is a tool that is built to aid in the air transportation management process through the power of advancing technologies and bettering user experience. NTMOs of aMaize will find themselves instead of navigating across 57+ distinct platforms to implement an AFP, they will have the ability to focus their tasks directly on the aMaize interface, not having their workflow being scattered and distracted by jumping through the numerous applications. To see how aMaize impacts and improves upon the NTMO's work experience and how it connects with air transportation management, we outlined a user persona that directly will be impacted by aMaize. Our primary persona is an individual who has been  exposed to aviation and kickstarted her career working at the local fixed-base operator (FBO). They then moved to the FAA to pursue the dream of solving aviation puzzles as a Traffic Control Specialist and is now ready to move up the ranks to a TMO. As a new TMO being onboarded into FMDS services, they struggle to adapt to the current interface, coupled with the breadth of traffic they have to manage. Therefore, they are looking for something that ties their disparate tasks together into one, easy-to-navigate interface.

% To better replicate the NTMS workflow, we included functionalities for Miles-In-Trail (MIT), Ground-Delay-Programs (GDPs), and Ground Stops (GS). By maintaining the core structure of aMaize, our team has performed research into these TMIs to determine the best structure for these workflows.

%How did this wireframe connect with air transportation management :NTMOs will use this instead of the 57 TFMS applications; For a detailed example, reference our CDR technical document page X (User story?); How aMaize might adapt to MITs, GDPs, Ground Stops (Our core functionalities are translatable to other TMIs and we also demonstrated in our data card that we can add other TMIs and we can build upon that)

%We will discuss some of the implications of our FMDS-based GUI. 
Our interface allows NTMS to work within one interface to accomplish their ATM tasks, rather than navigating 50+ different applications, improving workplace efficiency, decreasing cognitive load, and decreasing chance of user error or distraction. While our GUI is tailored to the AFP workflow, the three \textit{Core functionalities} can be adapted to other TMIs, including MITs, GDPs, and ground stops, as each TMI requires some form of evaluation, creation, and monitoring (see Section \ref{sec:Iteration 3}). 

%To facilitate integration, we introduced a feature to our \textit{Data Cards} that enables NTMS to easily include other TMIs by clicking the \enquote{+} button.
% how do we actually get this implemented
%There are several steps that need to be taken to make this interface fully functional. Front-end developers will first need to build out the interface and back-end developers will need to  occur: connecting SWIM APIs to the interface, including machine learning capabilities (e.g. automation-assisted NTML logging, meeting scheduling), and addressing cybersecurity concerns. Full-stack developers will be included throughout this process, ensuring the user experience is maintained.

There are several steps that need to be taken to make this interface fully functional. Front-end developers will first need to build out the interface and back-end developers will need to connect to SWIM APIs and integrate with machine learning capabilities that aid users in completing tasks (e.g., automation-assisted NTML logging, meeting scheduling), and addressing cybersecurity concerns. Full-stack developers will be included throughout this process, ensuring the application is fully integrated.

% future works from FAA standpoint 
The FAA plans to transition from TFMS to FMDS over the next five years, with a focus on web-based architectures for several FMDS applications \cite{xxx}. %To achieve this transition by Fall 2028, the FAA will need to develop data streams required for summary statistics and data visualizations. 
Given this, we note that cybersecurity risks should be considered, and integrated within the full-stack development process of FMDS. %Furthermore, with the FAA planning on a web-based architecture for several FMDS applications, they will have to consider cybersecurity risks. %Managing the \enquote{safest, busiest and most complex airspace system in the world,} safety measures must exist to protect FMDS against any potential cybersecurity threat (e.g. protecting APIs that power SWIM data and the internalized Collaboration Feature). However, the FAA can refer to existing literature or even web-based TFMS applications to mitigate these risks.
Additionally, our %The FAA would not be the only beneficiary of our GUI, as a 
user-centered FMDS interface can also be of great benefit to air carriers, by enhancing the CDM process. Specifically, having access to an improved TSD-style map where NAS constraints are identified, plus improved NTML functionalities, allow airlines to be more informed about potential ATM actions that the ATCSCC is considering.

% that can improve CDM and minimize delays to aircraft brings significant savings to air carriers, as discussed in Section \ref{sec:lit_review}. Having access to an improved TSD-style map where NAS constraints are identified and an improved NTML functionality allows airlines to be more informed on potential ATM actions the ATCSCC is considering. Summary statistics and improved data visualizations via redesigned FSM graphs allow airlines to be more informed about the impact of different TMIs. FSM in particular is heavily used by airlines such as DL (see Section \ref{sec:Airlines}) to understand demand-capacity imbalances and we anticipate that our redesigned FSM could be a key tool for influencing air carriers' ATM strategy.
